Combined analysis of charm-quark fragmentation-fraction measurements

A summary of measurements of the fragmentation of charm quarks into a specific hadron is given. Measurements performed in photoproduction and deep inelastic scattering in $e^{\pm}p$, $pp$ and $e^+e^-$ collisions are compared, using up-to-date branching ratios. Within uncertainties, all measurements agree, supporting the hypothesis that fragmentation is independent of the specific production process. Averages of the fragmentation fractions over all measurements are presented. The average has significantly reduced uncertainties compared to individual measurements.

==> Makefile <==
latexfile=FFC
newname?=FFC
STYLE=arxiv

LATEX=latex -halt-on-error -shell-escape
BIBTEX=bibtex


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex
endif


all: $(latexfile)-$(STYLE).pdf

tar:  Makefile $(figures) $(constanttables) $(tables) $(latexfile).bst $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	mkdir -p TAR/Figures
	mkdir -p TAR/Tables
	mkdir -p TAR/ConstantTables
	cp Makefile  $(latexfile).bst $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex    $(STYLE_SPECIFIC_FILES) TAR
	cp $(constanttables) TAR/ConstantTables
	cp $(tables) TAR/Tables
	cp $(figures) TAR/Figures
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif
	
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
	mv TAR/$(latexfile)-fig.tex TAR/$(newname)-fig.tex
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -f $(newname).zip
	cd TAR; zip -r ../$(newname).zip  ./*
	rm -rf TAR


figures=Figures/figure0.eps  Figures/figure0.pdf\
        Figures/figure1.eps  Figures/figure1.pdf 
tables=Tables/constants.txt Tables/constants_lhcb13.txt\
       Tables/ee10_tab.txt Tables/eez0_tab.txt Tables/heradis_tab.txt\
       Tables/heraphp_tab.txt Tables/lhcb_tab.txt Tables/average_tab2.txt\
       Tables/average_cov.txt Tables/excited_tab.txt Tables/pdg_tab.txt
constanttables=ConstantTables/pp_ALICE_7TeV.txt ConstantTables/pp_ATLAS_7TeV.txt\
               ConstantTables/av_David.txt ConstantTables/pp_CDF_2TeV.txt


$(latexfile)-$(STYLE).dvi :  $(figures) $(constanttables) $(tables) $(latexfile).bst\
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex   $(STYLE_SPECIFIC_FILES)
	
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)

$(latexfile)-$(STYLE).pdf : $(latexfile)-$(STYLE).ps
	ps2pdf -dUseCIEColor -dPDFSETTINGS=/printer -sPAPERSIZE=a4  $(latexfile)-$(STYLE).ps $(latexfile)-$(STYLE).pdf

ps : $(latexfile)-$(STYLE).ps 

pdf : $(latexfile)-$(STYLE).pdf
$(latexfile)-$(STYLE).ps : $(latexfile)-$(STYLE).dvi
	dvips -Ppdf -t a4 $(latexfile)-$(STYLE)


$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		cat $$a |aspell  list --add-tex-command="app p" --add-tex-command="label p" --add-tex-command="eq p" --add-tex-command="usetikzlibrary p" --add-tex-command="sect p" --add-tex-command="fig p" --add-tex-command="tab p"  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB ;\
		done

		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
#		aspell   --add-tex-command="label p" --add-tex-command="usetikzlibrary p" --add-tex-command="sect p" --add-tex-command="fig p" --add-tex-command="tab p"  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB -c $$a ;\
		done

clean :
	rm -f $(latexfile)-papers.tex
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm


	

